Algorithmic correspondence and analytic rules

We introduce the algorithm MASSA which takes classical modal formulas in input, and, when successful, effectively generates: (a) (analytic) geometric rules of the labelled calculus G3K, and (b) cut-free derivations (of a certain `canonical' shape) of each given input formula in the geometric labelled calculus obtained by adding the rule in output to G3K. We show that MASSA successfully terminates whenever its input formula is a (definite) analytic inductive formula, in which case, the geometric axiom corresponding to the output rule is, modulo logical equivalence, the first-order correspondent of the input formula. In proving the correctness of MASSA, we also show that the algorithm for the elimination of second-order quantifiers SCAN is complete with respect to the class of inductive analytic formulas. Finally, we show how our algorithm can be extended to the class of inductive formulas and to modal logic with quantifiers.

==> macros.tex <==
\def\aol{\rule[0.5865ex]{1.38ex}{0.1ex}}
\def\AOL{\rule[0.65ex]{1.45ex}{0.1ex}}

\newcommand{\FH}{\hat{f}}
\newcommand{\FHp}{\hat{f}_{1}}
\newcommand{\FHs}{\hat{f}_{2}}
\newcommand{\FC}{\check{f}}
\newcommand{\GH}{\hat{g}}
\newcommand{\GHp}{\hat{g}_{1}}
\newcommand{\GHs}{\hat{g}_{2}}
\newcommand{\GC}{\check{g}}

\newcommand{\FHS}{\hat{f}^{\,\sharp}}
\newcommand{\FCS}{\check{f}^{\,\sharp}}
\newcommand{\GHF}{\hat{g}^{\,\flat}}
\newcommand{\GCF}{\check{g}^{\,\flat}}

%Multiplicative Operational connectives
\newcommand{\mtop}{1}
\newcommand{\mbot}{0}
\newcommand{\mand}{\otimes}
\newcommand{\mdlarr}{\varobslash}
\newcommand{\mdrarr}{\varoslash}
\newcommand{\mor}{\oplus}
\newcommand{\mrarr}{\,\,\backslash\,\,}
\newcommand{\mlarr}{\,\,\slash\,\,}
%
%Multiplicative Structural connectives
\newcommand{\MTOP}{\hat{1}}
\newcommand{\MBOT}{\check{0}}
\newcommand{\MAND}{\,\hat{\otimes}\,}
\newcommand{\MRARR}{\,\,\check{\backslash}\,\,}
\newcommand{\MLARR}{\,\check{\slash}\,}
\newcommand{\MOR}{\,\check{\oplus}\,}
\newcommand{\MDLARR}{\,\hat{\varobslash}\,}
\newcommand{\MDRARR}{\,\hat{\varoslash}\,}

%Distributive Lattice
%Operational Connectives
\newcommand{\aneg}{\ensuremath{\neg}\xspace}
\newcommand{\aatop}{\ensuremath{\top}\xspace}
\newcommand{\abot}{\ensuremath{\bot}\xspace}
\newcommand{\aand}{\ensuremath{\wedge}\xspace}
\newcommand{\aor}{\ensuremath{\vee}\xspace}
\newcommand{\ararr}{\ensuremath{\rightarrow}\xspace}
\newcommand{\alarr}{\ensuremath{\leftarrow}\xspace}
\newcommand{\adrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
\newcommand{\adlarr}{\ensuremath{\rotatebox[origin=c]{180}{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}\xspace}
%
%Structural Connectives
\newcommand{\ANEG}{\ensuremath{\:\tilde{\neg}}\xspace}
\newcommand{\ATOP}{\hat{\top}}
\newcommand{\ABOT}{\ensuremath{\check{\bot}}\xspace}
\newcommand{\AAND}{\ensuremath{\:\hat{\wedge}\:}\xspace}
\newcommand{\AOR}{\ensuremath{\:\check{\vee}\:}\xspace}
\newcommand{\ARARR}{\ensuremath{\:\check{\rightarrow}\:}\xspace}
\newcommand{\ALARR}{\ensuremath{\:\check{\leftarrow}\:}\xspace}
\newcommand{\ADRARR}{\ensuremath{\hat{{\:{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\:}}}\xspace}
\newcommand{\ADLARR}{\ensuremath{\:\hat{\rotatebox[origin=c]{180}{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}\:}\xspace}

%Unary Modalities
%Operational connectives
\newcommand{\wbox}{\ensuremath{\Box}\xspace}
\newcommand{\wdia}{\ensuremath{\Diamond}\xspace}
\newcommand{\bbox}{\ensuremath{\blacksquare}\xspace}
\newcommand{\bdia}{\ensuremath{\Diamondblack}\xspace}
\newcommand{\bcirc}{\ensuremath{{\bullet}}\xspace}
\newcommand{\bboxdot}{\ensuremath{\boxdot}\xspace}
\newcommand{\bdialoz}{\ensuremath{\blacklozenge}\xspace}
%Structural connectives
\newcommand{\WBOX}{\ensuremath{\check{\Box}}\xspace}
\newcommand{\WDIA}{\ensuremath{\hat{\Diamond}}\xspace}
\newcommand{\BBOX}{\ensuremath{\check{\blacksquare}}\xspace}
\newcommand{\BDIA}{\ensuremath{\hat{\Diamondblack}}\xspace}
\newcommand{\WCIR}{\ensuremath{\tilde{{\circ}}}\xspace}
\newcommand{\BCIR}{\ensuremath{\tilde{{\bullet}}}\xspace}


%%% Abbreviazioni %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\f}{\overline}

\newcommand{\ls}{\lbrack}
\newcommand{\rs}{\rbrack}
\newcommand{\lc}{\langle}
\newcommand{\rc}{\rangle}

%LETTERS
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\Po}{\mathcal{P}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\mvspec}{\mathrm{mvspec}}

%SYMBOLS
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\leftmapsto}{\mathbin{\reflectbox{$\mapsto$}}}
\newcommand{\embeds}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\op}{\mathrm{op}}
\newcommand{\vp}{\overline{p}}
\newcommand{\vq}{\overline{q}}
\newcommand{\va}{\overline{a}}
\newcommand{\vb}{\overline{b}}

\newcommand{\ox}{\overline{x}}
\newcommand{\oy}{\overline{y}}
\newcommand{\oz}{\overline{z}}
\newcommand{\oX}{\overline{X}}
\newcommand{\oa}{\overline{a}}
\newcommand{\ob}{\overline{b}}
\newcommand{\ovlc}{\overline{c}}
\newcommand{\oone}{\overline{1}}
\newcommand{\opar}{\overline{\partial}}
\newcommand{\ophi}{\overline{\phi}}
\newcommand{\opsi}{\overline{\psi}}
\newcommand{\oga}{\overline{\gamma}}

\newcommand{\pspBox}{PSPIA$^{\Box}$}
\newcommand{\pspDia}{PSPIA$^{\Diamond}$}
\newcommand{\pspLhd}{{PSPIA$^{{\lhd}}$}}
\newcommand{\pspRhd}{{PSPIA$^{{\rhd}}$}}
\newcommand{\isBox}{IS$^{\Box}$}
\newcommand{\isDia}{IS$^{\Diamond}$}
\newcommand{\isLhd}{{IS$^{{\lhd}}$}}
\newcommand{\isRhd}{{IS$^{{\rhd}}$}}
\newcommand{\ifBox}[1]{IF$^{\Box}_{#1}$}
\newcommand{\ifDia}[1]{IF$^{\Diamond}_{#1}$}
\newcommand{\ifLhd}{{IF$^{{\lhd}}$}}
\newcommand{\ifRhd}{{IF$^{{\rhd}}$}}
\newcommand{\If}{\Rightarrow}

\newcommand{\diamdot}{\Diamond\!\!\!\cdot\ }
\newcommand{\lhddot}{{\lhd}\!\!\cdot\ }
\newcommand{\rhddot}{{\rhd}\!\!\!\cdot\ }
\newcommand{\diamdotland}{\Diamond\!\!\!\!\cdot\ }
\newcommand{\lhddotland}{{\lhd}\!\!\!\!\cdot\ }
\newcommand{\rhddotland}{{\rhd}\!\!\!\!\cdot\ }
\newcommand{\diamdotb}{\Diamondblack\!\!\!{\color{white}{\cdot\ }}}
\newcommand{\boxdotb}{\blacksquare\!\!\!{\color{white}{\cdot\ }}}
\newcommand{\lhddotb}{{\blacktriangleleft}\!\!{\color{white}{\cdot\ }}}
\newcommand{\rhddotb}{{\blacktriangleright}\!\!\!{\color{white}{\cdot\ \ }}}
\newcommand{\nomh}{\mathbf{h}}
\newcommand{\nomi}{\mathbf{i}}
\newcommand{\nomj}{\mathbf{j}}
\newcommand{\nomk}{\mathbf{k}}
\newcommand{\noml}{\mathbf{l}}
\newcommand{\cnomm}{\mathbf{m}}
\newcommand{\cnomn}{\mathbf{n}}
\newcommand{\cnomo}{\mathbf{o}}
%\renewcommand{\hat}{\widehat}
\newcommand{\id}{\mathrm{id}}
\newcommand{\gen}[1]{\langle #1 \rangle}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\dual}{\partial}
\newcommand{\isom}{\cong}
\newcommand{\limp}{\rightarrow}
\newcommand{\diam}{\Diamond}
%\renewcommand{\i}{\mathbf{i}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\ca}{A^\delta}
\newcommand{\blhd}{\blacktriangleleft}
\newcommand{\brhd}{\blacktriangleright}
\newcommand{\bs}{\Box_\sigma}
\newcommand{\dimp}{\Diamond_\pi}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\rhu}{\rightharpoonup}
\newcommand{\lhu}{\leftharpoonup}
\newcommand{\bba}{\mathbb{A}}
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbas}{A^{\delta}}
\newcommand{\kbbas}{K(A^\delta)}
\newcommand{\obbas}{O(A^\delta)}
\newcommand{\jty}{J^{\infty}}
\newcommand{\mty}{M^{\infty}}
\newcommand{\AATOP}{\hat{\top}}
\newcommand{\fs}{\ensuremath{f^\sharp}\xspace}
\newcommand{\gf}{\ensuremath{g^\flat}\xspace}

\newcommand{\marginnote}[1]{\marginpar{\raggedright\tiny{#1}}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle ,draw, minimum size=3.5mm, inner sep=0pt] (char) {#1};}}

\newcommand*\dcircled[1]{\tikz[baseline=-3pt]{
		\node[shape=circle ,draw, minimum size=3.5mm, inner sep=0pt] (char) {#1};}}

\tikzset{
	treenode/.style = {align=center, inner sep=0pt, text centered},
	Ske/.style = {treenode, ellipse, double, draw=black,
		minimum width=6pt, thick},% arbre rouge noir, noeud noir
	PIA/.style = {treenode, ellipse, black, draw=black,
		minimum width=6pt},% arbre rouge noir, noeud rouge
	Crit/.style = {treenode, rectangle, draw=black,
		minimum width=0.5em, minimum height=0.5em}% arbre rouge noir, nil
}

%
%THEOREM STYLES

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem*{thmstar}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{fact}[thm]{Fact}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{notation}[thm]{Notation}

\theoremstyle{definition}
\newtheorem{dfn}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{exa}[thm]{Example}
\newtheorem{example}[thm]{Example}

\newtheorem{exs}[thm]{Example}
\newtheorem{rem}[thm]{Remark}
\newtheorem{claim}[thm]{Claim}
\newtheorem{remark}[thm]{Remark}

\renewcommand{\labelenumi}{\arabic{enumi}.}

%%Derivations
\def\fCenter{{\mbox{$\ \vdash\ $}}}
\def\ffCenter{{\mbox{$\overline{\vdash}$}}}
\def\fcenter{{\mbox{\ }}}
\EnableBpAbbreviations

%Abbreviations Tabular, Size, Marginnote, Equations
\newcommand{\fns}{\footnotesize}
\newcommand{\mc}{\multicolumn}
\newcommand{\mr}{\multirow}
%
\newcommand{\redbf}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\bfred}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
%
\newcommand{\marginred}[1]{\marginpar{\raggedright\tiny{\red{#1}}}}
\newcommand{\marginredbf}[1]{\marginpar{\raggedright\tiny{\redbf{#1}}}}
%
\newcommand{\commment}[1]{}
%
\numberwithin{equation}{section}

%%%

%%%Propositional connectives (old)
\def\pRA{\mbox{$\,\,{\AOL{\mkern-0.4mu{\rotatebox[origin=c]{-90}{\raisebox{0.12ex}{$\pAND$}}}}}\,\,$}}
%
\def\pDRA{\mbox{$\,\,{\rotatebox[origin=c]{-90}{\raisebox{0.12ex}{$\pAND$}}{\mkern-1mu\AOL}}\,\,$}}
%
\def\pdra{\mbox{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}
\def\pdla{\mbox{\rotatebox[origin=c]{180}{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}}
%
\newcommand{\pneg}{\neg}
\newcommand{\pNEG}{\mbox{\boldmath{${\neg\,}$}}}
\newcommand{\pNEGL}{\mbox{{\boldmath{$\neg$}}$_L$\,}}
\newcommand{\pNEGR}{\mbox{{\boldmath{$\neg$}}$_R$\,}}
%
\newcommand{\pand}{\wedge}
\newcommand{\pAND}{\mbox{$\,\bigwedge\,$}}
%
\newcommand{\por}{\vee}
\newcommand{\pOR}{\mbox{$\,\bigvee\,$}}
%
\newcommand{\pra}{\rightarrow}
\newcommand{\plra}{\leftrightarrow}
\newcommand{\pla}{\leftarrow}
%%%

\newcommand{\cfDLE}{\underline{D.LE}}
\newcommand{\cfDDLE}{\underline{D.DLE}}

%colours
%blue
\newcommand{\bp}{\textcolor{blue}{p}}
\newcommand{\bx}{\textcolor{blue}{x}}
\newcommand{\bu}{\textcolor{blue}{u}}
\newcommand{\bz}{\textcolor{blue}{z}}
\newcommand{\bw}{\textcolor{blue}{w}}
\newcommand{\bi}{\textcolor{blue}{i}}
\newcommand{\bj}{\textcolor{blue}{j}}
\newcommand{\bk}{\textcolor{blue}{k}}
\newcommand{\bh}{\textcolor{blue}{h}}
\newcommand{\obp}{\overline{\textcolor{blue}{p}}}
\newcommand{\obx}{\overline{\textcolor{blue}{x}}}
\newcommand{\obz}{\overline{\textcolor{blue}{z}}}
%red
\newcommand{\rrq}{\textcolor{red}{q}}
\newcommand{\ru}{\textcolor{red}{u}}
\newcommand{\ry}{\textcolor{red}{y}}
\newcommand{\rz}{\textcolor{red}{z}}
\newcommand{\rw}{\textcolor{red}{w}}
\newcommand{\ri}{\textcolor{red}{i}}
\newcommand{\rj}{\textcolor{red}{j}}
\newcommand{\rk}{\textcolor{red}{k}}
\newcommand{\rh}{\textcolor{red}{h}}
\newcommand{\orq}{\overline{\textcolor{red}{q}}}
\newcommand{\ory}{\overline{\textcolor{red}{y}}}
\newcommand{\orw}{\overline{\textcolor{red}{w}}}
%
%blue
\newcommand{\ba}{\textcolor{blue}{\alpha}}
\newcommand{\oba}{\overline{\textcolor{blue}{\alpha}}}
\newcommand{\bpsi}{\textcolor{blue}{\psi}}
\newcommand{\bPsi}{\textcolor{blue}{\Psi}}
\newcommand{\obpsi}{\overline{\textcolor{blue}{\psi}}}
\newcommand{\obPsi}{\overline{\textcolor{blue}{\Psi}}}
\newcommand{\bgamma}{\textcolor{blue}{\gamma}}
\newcommand{\bGamma}{\textcolor{blue}{\Gamma}}
\newcommand{\bS}{\textcolor{blue}{S}}
\newcommand{\bsigma}{\textcolor{blue}{\sigma}}
%red
\newcommand{\rb}{\textcolor{red}{\beta}}
\newcommand{\orb}{\overline{\textcolor{red}{\beta}}}
\newcommand{\rxi}{\textcolor{red}{\xi}}
\newcommand{\rXi}{\textcolor{red}{\Xi}}
\newcommand{\orxi}{\overline{\textcolor{red}{\xi}}}
\newcommand{\orXi}{\overline{\textcolor{red}{\Xi}}}
\newcommand{\rvarphi}{\textcolor{red}{\varphi}}
\newcommand{\rVarphi}{\textcolor{red}{\Phi}}
\newcommand{\rdelta}{\textcolor{red}{\delta}}
\newcommand{\rDelta}{\textcolor{red}{\Delta}}
\newcommand{\rU}{\textcolor{red}{U}}
\newcommand{\rtau}{\textcolor{red}{\tau}}


%non normal modal logic macros

\newcommand{\abla}{\nabla}
%\newcommand{\land}{\wedge}

\newcommand{\XDIANU}{\ensuremath{\langle\hat{\nu}\rangle}\xspace}
\newcommand{\xdianu}{\ensuremath{\langle\nu\rangle}\xspace}

\newcommand{\DBOXNI}{\ensuremath{[\check\ni]}\xspace}
\newcommand{\dboxni}{\ensuremath{[\ni]}\xspace}

\newcommand{\XBOXNUC}{\ensuremath{[\check{\nu^c}]}\xspace}
\newcommand{\xboxnuc}{\ensuremath{[\nu^c]}\xspace}

\newcommand{\XDIAIN}{\ensuremath{\langle\hat{\in}\rangle}\xspace}
\newcommand{\xdiain}{\ensuremath{\langle\in\rangle}\xspace}

\newcommand{\XAND}{\ensuremath{\:\hat{\wedge}\:}\xspace}
\newcommand{\xand}{\ensuremath{\wedge}\xspace}

\newcommand{\xor}{\ensuremath{\vee}\xspace}
\newcommand{\XOR}{\ensuremath{\:\check{\vee}\:}\xspace}

\newcommand{\DDIANNI}{\ensuremath{\langle\hat{\not\ni}\rangle}\xspace}
\newcommand{\ddianni}{\ensuremath{\langle\not\ni\rangle}\xspace}

\newcommand{\vd}{\ \,\textcolor{black}{\vdash}\ \,}

==> packages.tex <==
\usepackage{lscape}
\usepackage{pdflscape}


\usepackage{stmaryrd}
\usepackage{mathdots}

%\usepackage[greek.ancient,english]{babel}
%\usepackage[greek,english]{babel}
\usepackage[geometry]{ifsym}
\usepackage{cmll}

\usepackage{comment}
%\usepackage{proof}

%\usepackage{eucal}
\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{mathptmx}
\usepackage{mathrsfs}

\usepackage{color}
\usepackage{xspace}
\usepackage{bussproofs}
\EnableBpAbbreviations

%\usepackage[single]{accents}
%\usepackage{graphicx}
%\usepackage{amscd}

%\usepackage{unicode-math}
\usepackage{mathtools}
%\setmathfont{XITS math}


%\usepackage{amssymb,amsmath}
%%%\usepackage{mathptmx}
%\usepackage{mathrsfs}


%\usepackage{tikz}



\usepackage{bpextra}


\usepackage{enumerate}

\usepackage{centernot}


%\usepackage{mathtools}



\usepackage{hyperref}

\usepackage{cleveref}

%\usepackage{relsize}

\usepackage{caption}

\usepackage{multirow}

%\usepackage{multicol}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\arraybackslash}p{#1}}




%\usepackage{graphics}
\usepackage{color}
\usepackage{cancel}
%\usepackage{stmaryrd}
%%\usepackage{amssymb,amsmath}
%\usepackage{amsthm}
%[nointegrals]
%\usepackage{proof}
\usepackage{verbatim,cmll}
\usepackage{setspace}
\usepackage{lscape}
\usepackage{latexsym,relsize}
%\usepackage{amscd}
\usepackage{multicol}
%\usepackage{bussproofs}
%\EnableBpAbbreviations

\usepackage[position=top]{subfig}
\usepackage{leqno}
\usepackage{tikz}

\usepackage{txfonts}

%\usepackage{authblk}
\usepackage{multicol}
\usetikzlibrary{arrows}
\usetikzlibrary{matrix}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes}
%\usepackage[bb=boondox]{mathalfa}
%\usepackage{enumerate}

